Towards Better Text Understanding and Retrieval through Kernel Entity Salience Modeling

This paper presents a Kernel Entity Salience Model (KESM) that improves text understanding and retrieval by better estimating entity salience (importance) in documents. KESM represents entities by knowledge enriched distributed representations, models the interactions between entities and words by kernels, and combines the kernel scores to estimate entity salience. The whole model is learned end-to-end using entity salience labels. The salience model also improves ad hoc search accuracy, providing effective ranking features by modeling the salience of query entities in candidate documents. Our experiments on two entity salience corpora and two TREC ad hoc search datasets demonstrate the effectiveness of KESM over frequency-based and feature-based methods. We also provide examples showing how KESM conveys its text understanding ability learned from entity salience to search.

==> archive/Evaluation.tex <==

\begin{table*}[t]
\centering
\caption{
Entity salience prediction performances on the New York Times corpus and the Semantic Scholar corpus.
(E), (W), and (S) mark the component used by \texttt{KESM}: entity kernels, word kernels, and semantic memory.   \texttt{KESM} is the full model.
Relative performances over \texttt{LeToR} are shown in the percentages. W/T/L are the number of documents a method improves, does not change, and hurts, also compared to \texttt{LeToR}. $\dagger$, $\ddagger$, $\mathsection$, and $\mathparagraph$ mark the statistically significant improvements over \texttt{Frequency}$^\dagger$, \texttt{Page Rank}$^\ddagger$, \texttt{LeToR}$^\mathsection$, and \texttt{KESM (E)}$^\mathparagraph$.
Best results are marked \textbf{bold}.
\label{tab:overall_salience}
}

\begin{tabular}{l|lr|lr|lr|lr|c}
\hline \hline
\multicolumn{10}{c}{\textbf{New York Times}} \\ \hline
\bf{Method}& \multicolumn{2}{c|}{\bf{Precision@1}}& \multicolumn{2}{c|}{\bf{Precision@5}}& \multicolumn{2}{c|}{\bf{Recall@1}}& \multicolumn{2}{c|}{\bf{Recall@5}}&\bf{W/T/L}\\ \hline
\texttt{Frequency}
 & ${0.5840}$ & $ -8.53\%  $

 & ${0.4065}$ & $ -11.82\%  $

 & ${0.0781}$ & $ -11.92\%  $

 & ${0.2436}$ & $ -14.44\%  $

& 5622/38813/19154

\\
\texttt{Page Rank}
 & ${0.5845}^{\dagger }$ & $ -8.46\%  $

 & ${0.4069}^{\dagger }$ & $ -11.73\%  $

 & ${0.0782}^{\dagger }$ & $ -11.80\%  $

 & ${0.2440}^{\dagger }$ & $ -14.31\%  $

& 5655/38841/19093

\\ \hline
\texttt{LeToR}
 & $0.6385$ & --  & $0.4610$ & --  & $0.0886$ & --  & $0.2848$ & --  & --/--/--\\
 \hline
\texttt{KESM (E)}
 & ${0.6470}^{\dagger \ddagger \mathsection }$ & $ +1.33\%  $

 & ${0.4782}^{\dagger \ddagger \mathsection }$ & $ +3.73\%  $

 & ${0.0922}^{\dagger \ddagger \mathsection }$ & $ +4.03\%  $

 & ${0.3049}^{\dagger \ddagger \mathsection }$ & $ +7.05\%  $

& 19778/27983/15828

\\
\texttt{KESM (ES)}
 & ${0.6528}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +2.24\%  $

 & ${0.4769}^{\dagger \ddagger \mathsection }$ & $ +3.46\%  $

 & ${0.0920}^{\dagger \ddagger \mathsection }$ & $ +3.82\%  $

 & ${0.3026}^{\dagger \ddagger \mathsection }$ & $ +6.27\%  $

& 18619/29973/14997

\\
\texttt{KESM (EW)}
 & ${0.6767}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +5.98\%  $

 & ${0.5018}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +8.86\%  $

 & ${0.0989}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +11.57\%  $

 & ${0.3277}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +15.08\%  $

& 22805/26436/14348

\\ \hline

\texttt{KESM}
 & $\bf{0.6866}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +7.53\%  $

 & $\bf{0.5080}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +10.21\%  $

 & $\bf{0.1010}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +13.93\%  $

 & $\bf{0.3335}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +17.10\%  $

& 23290/26883/13416

\\ \hline \hline

\end{tabular}

\vspace{0.2cm}

\begin{tabular}{l|lr|lr|lr|lr|c}
\hline \hline
\multicolumn{10}{c}{\textbf{Semantic Scholar}} \\ \hline
\bf{Method}& \multicolumn{2}{c|}{\bf{Precision@1}}& \multicolumn{2}{c|}{\bf{Precision@5}}& \multicolumn{2}{c|}{\bf{Recall@1}}& \multicolumn{2}{c|}{\bf{Recall@5}}&\bf{W/T/L}\\ \hline

\texttt{Frequency}
& ${0.3944}$ & $ -9.99\%  $

 & ${0.2560}$ & $ -11.38\%  $

 & ${0.1140}$ & $ -12.23\%  $

 & ${0.3462}$ & $ -13.67\%  $

& 11155/64455/24390
 \\
\texttt{Page Rank}
& ${0.3946}^{\dagger }$ & $ -9.94\%  $

 & ${0.2561}^{\dagger }$ & $ -11.34\%  $

 & ${0.1141}^{\dagger }$ & $ -12.11\%  $

 & ${0.3466}^{\dagger }$ & $ -13.57\%  $

& 11200/64418/24382

\\ \hline

\texttt{LeToR}
& $0.4382$ & --  & $0.2889$ & --  & $0.1299$ & --  & $0.4010$ & --  & --/--/-- \\ \hline

\texttt{KESM (E)}
& ${0.4793}^{\dagger \ddagger \mathsection }$ & $ +9.38\%  $

 & ${0.3192}^{\dagger \ddagger \mathsection }$ & $ +10.51\%  $

 & ${0.1432}^{\dagger \ddagger \mathsection }$ & $ +10.26\%  $

 & ${0.4462}^{\dagger \ddagger \mathsection }$ & $ +11.27\%  $

& 27735/56402/15863

\\
\texttt{KESM (ES)}
& ${0.4901}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +11.84\%  $

 & ${0.3161}^{\dagger \ddagger \mathsection }$ & $ +9.43\%  $

 & ${0.1492}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +14.91\%  $

 & ${0.4449}^{\dagger \ddagger \mathsection }$ & $ +10.95\%  $

& 28191/54084/17725

\\
\texttt{KESM (EW)}
 & ${0.5097}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +16.31\%  $

 & ${0.3311}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +14.63\%  $

 & ${0.1555}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +19.77\%  $

 & ${0.4671}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +16.50\%  $

& 32592/50428/16980

\\ \hline

\texttt{KESM}
 & $\bf{0.5169}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +17.96\%  $

 & $\bf{0.3336}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +15.47\%  $

 & $\bf{0.1585}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +22.09\%  $

 & $\bf{0.4713}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +17.53\%  $

& 32420/52090/15490

\\ \hline \hline
\end{tabular}

\end{table*}


\section{Evaluation Results}
The section first presents the overall evaluation results on the entity salience task and the ad hoc search task. Then it provide analyses about the advantages of modeling salience over counting frequency and case studies that demonstrate the connections between semantic text understanding and search accuracy.

\subsection{Entity Salience Performance}
%=====to discuss
	% KESM's individual components E, W, S
	% Table description
    % baseline performance
    	% Frequency, PR and LeToR
    % E VS PR, the gain of kernels    
    % +S: more stable and easier to converge
    % +W: another gains: we need word-entity duet
    % Full model: effectiveness and robustness
    
    % Compare the frequency performance, and the relative gains on the two data sets, lead to experiment 3.
%==================
The overall results in the entity salience task are in Table~\ref{tab:overall_salience}. 
All the relative performances (percentages) and document level \textbf{W}in/\textbf{T}ie/\textbf{L}oss are compared with \texttt{LeToR}, the feature-based state-of-the-art~\cite{dunietz2014new,dojchinovski2016crowdsourced}. 
% the word kernel votes, $\Phi(e, \mathbb{W})$, and the semantic memory that enriches the entity embedding with the description CNN. The groups of evidences used by  \texttt{KESM} versions are in the parentheses. \texttt{KESM (EWS)} is the full model.
Among the baselines, \texttt{Frequency} provides reasonable estimations of entity salience. 
The most frequent entity is often salient to the document; the Precision@1 is rather high, especially on New York Times. 
\texttt{Page Rank} does not perform well on both corpora. Although its embeddings are trained by the salience labels, it barely improves \texttt{Frequency}. 
\texttt{LeToR}, on the other hand, significantly improves both precision and recall of \texttt{Frequency}~\cite{dunietz2014new}, which is expected as it has much richer features from various sources.
% The Parsing and Coreference features provide more stable frequency counts, while position and embedding votes reflect entity importance. 

The full model \texttt{KESM} outperforms all baselines significantly. Its improvements over \texttt{LeToR} are more than $15\%$ on all evaluations, with the only exception on Precision@1 in New York Times. 
The improvements are also robust: About twice as many documents are improved (Win) than hurt (Loss). The neural salience model learned end-to-end is also rather different than manual features; \texttt{KESM} provided different salience estimations on half documents compared to \texttt{LeToR}.

Besides the full model \texttt{KESM}, its variants with partial evidence are also evaluated: Those marked with (E) include the entity kernels; those with (W) include word kernels; those with (S) incorporated semantic memories. All versions of \texttt{KESM} include the entity kernel group, which is the most essential evidence.

The full version (\texttt{KESM}) performs the best among all variations, showing that all components contributed.
Individually, \texttt{KESM (E)} outperforms all baselines. Compared to \texttt{Page Rank}, its only difference is that instead of raw cosine similarities,
\texttt{KESM (E)} uses kernel filters, which are much more powerful in modeling the interaction patterns and lead to completely different results than \texttt{Page Rank}~\cite{K-NRM}.
\texttt{KESM (EW)} always significantly outperform \texttt{KESM (E)}, showing the interactions with words are also important. 
However, the semantic memory (S) provides mixed impacts on the accuracy of \texttt{KESM}. A possible reason is that the Freebase descriptions might be too general and the training data is large enough for the entity embeddings to ``memorize'' the domain specific semantics. Nevertheless, we do find that adding the external semantics makes the model converges faster and more stably.


These results demonstrated that \texttt{KESM} is much more effective in modeling entity salience than counting frequency either directly (\texttt{Frequency}) or through complexed linguistic or semantic processes (\texttt{LeToR}). Section~\ref{sec:analysis} will further investigate the limitations of frequency signals and the advantages of modeling salience. 


\begin{table*}[t]
\centering
\caption{
Ad hoc search accuracy of \texttt{KESM} when used as ranking features in learning to rank.
Relative performances over \texttt{LeToR} are shown in the percentages. W/T/L are the number of queries a method improves, does not change, or hurts, compared with \texttt{LeToR}. $\dagger$, $\ddagger$, $\mathsection$, and $\mathparagraph$ mark the statistically significant improvements over \texttt{BOE-TagMe}$^\dagger$, \texttt{LeToR}$^\ddagger$, \texttt{ESR}$^\mathsection$, and \texttt{ESR+LeToR}$^\mathparagraph$. \texttt{Base} is the base retrieval model, which is SDM in ClueWeb09-B and language model in ClueWeb12-B13.
% All supervised ranking models used RankSVM with the same hyper-parameters and cross validation splits. 
Best results are marked \textbf{bold}.
\label{tab:overall_ranking}
}

\begin{tabular}{l|lr|lr|c||lr|lr|c}
\hline \hline
 & \multicolumn{5}{c||}{\bf{ClueWeb09-B}}
 & \multicolumn{5}{c}{\bf{ClueWeb12-B13}}
 \\ \hline 
\multicolumn{1}{c|}{\bf{Method}} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline

\texttt{Base}
 & ${0.2496}$ & $ -5.26\%  $

 & ${0.1387}$ & $ -10.20\%  $

& 62/38/100
 & ${0.1060}$ & $ -12.02\%  $

 & ${0.0863}$ & $ -6.67\%  $

& 35/22/43


\\
\texttt{BOE-TagMe}
 & ${0.2294}$ & $ -12.94\%  $

 & ${0.1488}$ & $ -3.63\%  $

& 74/25/101

 & ${0.1173}$ & $ -2.64\%  $

 & ${0.0950}$ & $ +2.83\%  $

& 44/19/37

\\
\hline

\texttt{LeToR}
 & $0.2635$ & --  & $0.1544$ & --  & --/--/--
 & $0.1205$ & --  & $0.0924$ & --  & --/--/--\\

\texttt{ESR}
 & ${0.2695}^{\dagger }$ & $ +2.30\%  $

 & ${0.1607}$ & $ +4.06\%  $

& 80/39/81
 & ${0.1166}$ & $ -3.22\%  $

 & ${0.0898}$ & $ -2.81\%  $

& 30/23/47

\\ \hline
\texttt{KESM}
 & ${0.2799}^{\dagger }$ & $ +6.24\%  $

 & ${0.1663}$ & $ +7.68\%  $

& 85/35/80
 & ${0.1301}^{\dagger \mathsection }$ & $ +7.92\%  $

 & $\bf{0.1103}^{\ddagger \mathsection \mathparagraph }$ & $ +19.35\%  $

& 43/25/32
\\
\hline
\hline
\texttt{ESR+LeToR}
 & ${0.2791}^{\dagger \ddagger }$ & $ +5.92\%  $

 & ${0.1613}$ & $ +4.46\%  $

& 91/34/75

 & ${0.1281}$ & $ +6.30\%  $

 & ${0.0951}$ & $ +2.87\%  $

& 45/24/31


\\
\texttt{KESM+LeToR}
 & $\bf{0.2993}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +13.58\%  $

 & $\bf{0.1797}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +16.38\%  $

& 98/35/67
& $\bf{0.1308}^{\dagger \mathsection }$ & $ +8.52\%  $

 & ${0.1079}^{\ddagger \mathsection \mathparagraph }$ & $ +16.77\%  $

& 43/23/34


\\
\hline \hline

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
\caption{
Ranking performances of \texttt{LeToR}, \texttt{ESR}, and \texttt{KESM} with title or body field individually.
Relative performances (percentages) and Win/Tie/Loss are calculated by comparing with \texttt{LeToR} on the same field.
$\dagger$ and $\ddagger$ mark the statistically significant improvements over \texttt{LeToR}$^\dagger$ and \texttt{ESR}$^\ddagger$, also on the same field.
Best results are marked \textbf{bold}.
\label{tab:field_ranking}
}

\begin{tabular}{l|lr|lr|c||lr|lr|c}
\hline \hline
 & \multicolumn{5}{c||}{\bf{ClueWeb09-B}}
 & \multicolumn{5}{c}{\bf{ClueWeb12-B13}}
 \\ \hline 
\multicolumn{1}{c|}{\bf{Method}} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline
\texttt{LeToR-Title}
  & ${0.2584}$ & $ -3.51\%  $

 & ${0.1460}$ & $ -5.16\%  $

& 83/48/69

 & ${0.1187}$ & $ +6.23\%  $

 & ${0.0894}$ & $ +3.14\%  $

& 41/23/36

 \\
\texttt{ESR-Title}
 & $0.2678$ & --  & $0.1540$ & --  & --/--/--
 & $0.1117$ & --  & $0.0867$ & --  & --/--/--

\\ \hline
\texttt{KESM-Title}
 & $\bf{0.2780}^{\dagger }$ & $ +3.81\%  $

 & $\bf{0.1719}^{\dagger \ddagger }$ & $ +11.64\%  $

& 91/46/63

 & $\bf{0.1199}$ & $ +7.36\%  $

 & $\bf{0.0923}$ & $ +6.42\%  $

& 35/28/37


\\ \hline \hline

\texttt{LeToR-Body}
 & ${0.2550}$ & $ +0.48\%  $

 & ${0.1427}$ & $ -3.44\%  $

& 80/46/74

 & ${0.1115}$ & $ +4.61\%  $

 & ${0.0892}$ & $ -3.51\%  $

& 36/30/34
\\
\texttt{ESR-Body}
& $0.2538$ & --  & $0.1478$ & --  & --/--/--
& $0.1066$ & --  & $0.0924$ & --  & --/--/--
\\ \hline
\texttt{KESM-Body}
  & $\bf{0.2795}^{\dagger \ddagger }$ & $ +10.13\%  $

 & $\bf{0.1661}^{\dagger \ddagger }$ & $ +12.37\%  $

& 96/39/65

  & $\bf{0.1207}^{\ddagger }$ & $ +13.25\%  $

 & $\bf{0.1057}^{\dagger \ddagger }$ & $ +14.44\%  $

& 43/24/33
\\
\hline \hline


\end{tabular}
\end{table*}



\subsection{Ranking Performance}

%===to discuss
	% overall performance
    	% KESM VS ESR
        % KESM+LeToR VS ESR+LeToR
        	%common set up
            %more additional information
        % shows that salience is better than frequency
        	% despite the knowledge transfer
     % per field performance
     	% no needs on title
        % better on body as expected, 10+\%
        % perform very differently with ESR, not only LeToR
        	% very different information

	% the task differences, the knowledge transfer, lead to the case study in experiment 4
Table~\ref{tab:overall_ranking} lists the evaluation results in the ad hoc search task.
The three supervised methods, \texttt{LeToR}, \texttt{ESR}, and \texttt{KESM}, all use the exact same learning to rank model (RankSVM) and only differ in their features.
% \texttt{LeToR} uses standard word-based features~\cite{xiong2017duet}; \texttt{ESR} uses the entity-based exact and soft match features using bag-of-entities (frequency-based) and pre-trained knowledge graph embeddings (TransE); \texttt{KESM} uses the normalized kernel votes that estimate the salience of query entities in the document. 
The effectiveness of \texttt{ESR} features and \texttt{KESM} features are also evaluated when combined with word-based features (\texttt{ESR+LeToR} and \texttt{KESM+LeToR}), which is a very common way to include new features in search engines.

On both ClueWeb09-B and ClueWeb12-B13, \texttt{KESM} features are more effective than both \texttt{LeToR} features and \texttt{ESR} features. On ClueWeb12-B13, \texttt{KESM} individually outperforms both supervised baselines significantly by $8-20\%$. On ClueWeb09-B, \texttt{KESM} provides more novel ranking signals and \texttt{KESM-LeToR} greatly improves the ranking accuracy than \texttt{ESR+LeToR}. The fusion on ClueWeb12-B13 (\texttt{KESM+LeToR}) is not as successful perhaps because of the limited ranking labels on ClueWeb12-B13.

Ranking is a complicated task with many factors influencing the final results. 
To better investigate the effectiveness of entity salience in search, we further evaluates the three supervised rankers on different document fields. Table~\ref{tab:field_ranking} lists the ranking accuracies of \texttt{LeToR}, \texttt{ESR}, and \texttt{KESM}, when only features from the document titles (\texttt{Title}) or the document body texts (\texttt{Body}) are used.

The per-field results reveal that the advantages of \texttt{KESM} are more significant and robust on the body field than on the title field.
Document titles are often short and more carefully written. Intuitively the handful entities mentioned in a title are all salient, despite spam.
The power of entity salience model is to find the importance of entities in document content---the \texttt{KESM} features learned from the New York Times corpus do reflect this semantic understanding capability on the body field features.

The W/T/L ratios in Table~\ref{tab:overall_ranking} and Table~\ref{tab:field_ranking} demonstrated that the entity salience features provide novel ranking signals.
Entity-oriented search was known to dramatically change the word-based rankings; both \texttt{ESR} and \texttt{KESM} perform rather differently with \texttt{LeToR} in Table~\ref{tab:overall_ranking}.
In addition, as shown in Table~\ref{tab:field_ranking}, the salience-based features also perform very different with \texttt{ESR}'s frequency-based features. Although both used the same entity annotations, \texttt{KESM} differs with \texttt{ESR} on $80\%$ queries and improved the majority of them.


A significant finding in our experiments is the connections of  entity salience  and  ad hoc search .
Entity salience was considered as a semantic text understanding task~\cite{dunietz2014new} while ad hoc search is a core information retrieval task.
The two tasks are different in many aspects: different focuses, different labels, different domains, and different applications. Despite these practical differences, 
the knowledge learned from entity salience labels are also effective on ad hoc search.
% Intuitively, the ability to better estimating entity salience improves the semantic text understanding in search engines which should lead to better search accuracy. 
Previously it is less common to see such connections between semantic text understanding tasks and information retrieval tasks.
Our case studies in Section~\ref{sec:case} will further discuss how \texttt{KESM} bridges the gap between semantic text understanding and search.






\begin{figure*}[t]
\centering
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\textwidth]{nyt_entity_dist.pdf}
\caption{New York Times \label{fig:nyt_dist}}
\end{subfigure}
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\textwidth]{s2_entity_dist.pdf}
\caption{Semantic Scholar \label{fig:s2_dist}}
\end{subfigure}
\caption{
The distribution of salient entities predicted by entity salience models and in the golden standard. The entities are binned by their frequencies in the testing data. The x-axes mark the percentile range of each group. The y-axes are the fraction of salient entities in each bin as predicted by the corresponding method.
The closer the predict salient entity distribution is to the golden standard, the more realistic an entity salience model is.
The histograms are ordered the same as the legends.
\label{fig:e_dist}
}
\end{figure*}


\begin{figure}[t]
\centering
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{nyt_doclen.pdf}
\caption{New York Times \label{fig:nyt_doclen}}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{s2_doclen.pdf}
\caption{Semantic Scholar \label{fig:s2_doclen}}
\end{subfigure}
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[width=\textwidth]{cw09_doclen.pdf}
% \caption{ClueWeb09-B \label{fig:cw09_doclen}}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
% \includegraphics[width=\textwidth]{cw12_doclen.pdf}
% \caption{ClueWeb12-B13 \label{fig:cw12_doclen}}
% \end{subfigure}

\caption{Performances on documents at different lengths.
Documents are partitioned based on their lengths (number of words).
The x-axes are the maximum length of the documents and their percentile of each group. 
The y-axes are the Precision@5 of corresponding methods.
The histograms are ordered the same as the legends.
\label{fig:doclen}
}
\end{figure}

\subsection{From Frequency To Salience}
\label{sec:analysis}
%====performance VS. doc length 
	%==unstable on short documents
    %==will not be sufficient at per document level anyway (can be on corpus level or large scale query log level)
    
%====estimation distribution
	%==frequency favors head entities
        %==biased
		%==less interesting for sure
This experiment provides two analyses that show the limitation of counting frequency and the advantage of modeling salience.


\textbf{Bias Towards Head Entities.}
The first drawback of frequency-based methods is that they are biased towards more frequent (head) entities. To demonstrate this effect, Figure~\ref{fig:e_dist} groups the entities based on their frequency in the corpus and plot the distribution of salience entities predicted by each method. 

The x-axes label the percentiles of each bin.
For example, $<0.1\%$ refers to the top $0.1\%$ most frequent entities. The distribution of predicted-salient entities is marked by the y-axes. The predicted-salient entities is the top k entities with highest salience scores predicted by a method, where k is the number of salient entities in the ground truth. \texttt{Golden Standard} is the ground truth.

In both datasets, entity salience follows the power law distribution. \texttt{Golden Standard} favors the head entities much more than the tail ones. However, the frequency-based methods are even more biased towards the head entities. More than $40\%$ of \texttt{Frequency}'s salience predictions go to top $0.1\%$ entities on New York Times and about $30\%$ on Semantic Scholar goes to the top $0.1\%$. They almost doubled the ground truth distributions. Such unrealistic bias towards the head entities limits the effectiveness of frequency-based methods and also their attractiveness---the selected entities are mostly common ones. 
In comparison, the distributions of \texttt{KESM} are much more closer to the ground truth. On Semantic Scholar the two are almost identical.

\textbf{Unreliable on Short Documents.}
The second drawback of frequency-based methods is that their reliability depends on the number of observations. Frequency signals can be very reliable at large scales. For example, the most frequent entities in a commercial search log or in a whole corpus probably reflect meaningful and stable trends. However, in each individual documents, the frequency signals might not be as reliable.

This analysis studies the performances of models on documents with different lengths in the entity salience task.
It groups the testing documents into five bins by their length (number of words). The performances of the frequency-based method (\texttt{Frequency}, feature-based method \texttt{LeToR}, and \texttt{KESM} in the five bins are plotted in Figure~\ref{fig:doclen}. The bins are ordered from short (left) to long (right) with their bin bounds and percentiles marked on the x-axes.

% In the entity salience task, 
There is a clear trend that the frequency signals are less reliable on shorter documents. As shown in Figure~\ref{fig:nyt_doclen} and Figure~\ref{fig:s2_doclen}, \texttt{Frequency} performs much worse on shorter documents, \texttt{LeToR} has a similar trend with \texttt{Frequency} as the majority of its signals are frequency-based, and the advantages on \texttt{KESM} are more significant on short documents.
% In ad hoc search, the correlations are less strong because the document length is the average of all candidate documents. Nevertheless, the improvements from \texttt{KESM} are again larger on shorter documents as shown in Figure~\ref{fig:cw09_doclen} and Figure~\ref{fig:cw12_doclen}.
On both datasets, even in the longest document bin where documents have thousands of words, the frequency-based method still under-performs salience-based method---counting frequency is not sufficient in modeling texts at the document level.







\begin{table*}[th]
\caption{Examples from queries that \texttt{KESM} improved or hurt, compared to \texttt{ESR}. 
Documents are selected from those that ESR and KESM disagreed.
The descriptions are manually written to reflect the main topics of the documents. 
\label{tab:eg}
}
\begin{tabular}{c|c|l|l}
\hline \hline
\multicolumn{4}{c}{\textbf{Cases that KESM Improved}} \\ \hline

\textbf{Query} & \textbf{Query Entities}  & \textbf{ESR Preferred Document}  & \textbf{KESM Preferred Document} \\ \hline 

\multirow{2}{*}{ER TV Show} & ``ER (TV Series)" & clueweb09-enwp02-22-20096 & clueweb09-enwp00-55-07707  \\
& ``TV Program" & ``List of films without article" & ``ER ( TV series ) - Wikipedia"  \\
\hline

\multirow{2}{*}{Wind Power
} &
\multirow{2}{*}{``Wind Power
''} 
& clueweb12-0200wb-66-32730 & clueweb12-0009wb-54-01932  \\

&  & ``Home solar power systems" & ``Wind energy | Alternative Energy HQ"  \\
\hline

Hurricane Irene  
 &
 ``Hurricane Irene"
& clueweb12-0705wb-49-04059 & clueweb12-0715wb-81-29281
 \\

Flooding in Manville NJ &  ``Flood";  ``Manville, NJ" & ``Disaster funding for Hurricane Irene" & ``Videos and news about Hurricane Irene"  \\
\hline
% \end{tabular}


% \begin{tabular}{c|c|l|l}
\hline \hline
\multicolumn{4}{c}{\textbf{Cases that KESM Hurt}} \\ \hline

% \textbf{Query} & \textbf{Query Entities}  & \textbf{ESR Preferred Document}  & \textbf{KESM Preferred Document} \\ \hline 

\multirow{2}{*}{Fickle Creek Farm
} &  ``Malindi Fickle"  & clueweb09-en0003-97-27345
 & clueweb09-en0005-66-00576
  \\
& ``Stream"; ``Farm" & ``Hotels near Fickle Creak" 
& ``List of breading farms"  \\
\hline

\multirow{3}{*}{Illinois State Tax
} &
``Illinois"; 
& clueweb09-enwp01-67-20725
 & clueweb09-en0011-23-05274
  \\

&  ``State government"; 
& ``Sales taxes in the United & ``Retirement-related general  \\

& ``Tax in the US"
& States, Wikipedia''
& purpose taxes by State''
\\

\hline

 \multirow{2}{*}{Battles in the Civil War}
 &
 ``Battles"
& clueweb09-enwp03-20-07742
 & clueweb09-enwp01-30-04139
 \\

 &  ``Civil War" & ``List of American Civil War battles" & ``List of wars in the Muslim world"  \\
\hline
\end{tabular}

\end{table*}

\subsection{From Text Understanding to Search}
\label{sec:case}


The last experiment provides case studies that demonstrate how \texttt{KESM} transfers the semantic text understanding learned from salience labels to search. We first picked the queries that \texttt{KESM-body} improved or hurt compared to \texttt{ESR-body}, Then we manually examined the top ranked documents that the two methods disagreed. The queries, query entities, and disagreed documents are listed in Table~\ref{tab:eg}. 

The improvements from \texttt{KESM} are mainly from its ability to promote documents that actually focus on the query entities. 
As shown in the top half of Table~\ref{tab:eg}, \texttt{KESM} promotes documents where the query entities are more salient: the Wikipedia page about ER TV show, a homepage about wind power, and the new article about the hurricane. On the other hand, \texttt{ESR}'s frequency-based ranking might be confused by web pages that list a lot of movies or only partially talk about the query topic; without modeling salience, it is hard to exclude those web pages because the query entities are also mentioned frequently in them.

Interestingly, many errors \texttt{KESM} made are also due to its emphasizes on query entities. When a query entity does not align with the information need, promoting documents about it is risky. As shown in the lower half of Table~\ref{tab:eg}, ``Malindi Fickle'' is a mistakenly linked query entity; ``Civil War'' in the Muslim world is in linked to the civil war in American, and the query ``Illinois State Tax'' is search for sales tax as designated by TREC by not ``Tax in the US''.


There are also other winning or losing scenarios and not all their causes are identifiable. Nevertheless, the main trend found in our case study is \texttt{KESM}'s ability to identify whether a document emphasis the query entities or not, which is exactly the motivation of the entity salience task. 





==> v1/Evaluation.tex <==

\begin{table*}[t]
\centering
\caption{
Entity salience prediction performances on the New York Times corpus and the Semantic Scholar corpus.
(E), (W), and (S) mark the component used by \texttt{KESM}: entity kernels, word kernels, and semantic memory.   \texttt{KESM} is the full model.
Relative performances over \texttt{LeToR} are shown in the percentages. W/T/L are the number of documents a method improves, does not change, and hurts, also compared to \texttt{LeToR}. $\dagger$, $\ddagger$, $\mathsection$, and $\mathparagraph$ mark the statistically significant improvements over \texttt{Frequency}$^\dagger$, \texttt{Page Rank}$^\ddagger$, \texttt{LeToR}$^\mathsection$, and \texttt{KESM (E)}$^\mathparagraph$.
Best results are marked \textbf{bold}.
\label{tab:overall_salience}
}

\begin{tabular}{l|lr|lr|lr|lr|c}
\hline \hline
\multicolumn{10}{c}{\textbf{New York Times}} \\ \hline
\bf{Method}& \multicolumn{2}{c|}{\bf{Precision@1}}& \multicolumn{2}{c|}{\bf{Precision@5}}& \multicolumn{2}{c|}{\bf{Recall@1}}& \multicolumn{2}{c|}{\bf{Recall@5}}&\bf{W/T/L}\\ \hline
\texttt{Frequency}
 & ${0.5840}$ & $ -8.53\%  $

 & ${0.4065}$ & $ -11.82\%  $

 & ${0.0781}$ & $ -11.92\%  $

 & ${0.2436}$ & $ -14.44\%  $

& 5622/38813/19154

\\
\texttt{Page Rank}
 & ${0.5845}^{\dagger }$ & $ -8.46\%  $

 & ${0.4069}^{\dagger }$ & $ -11.73\%  $

 & ${0.0782}^{\dagger }$ & $ -11.80\%  $

 & ${0.2440}^{\dagger }$ & $ -14.31\%  $

& 5655/38841/19093

\\ \hline
\texttt{LeToR}
 & $0.6385$ & --  & $0.4610$ & --  & $0.0886$ & --  & $0.2848$ & --  & --/--/--\\
 \hline
\texttt{KESM (E)}
 & ${0.6470}^{\dagger \ddagger \mathsection }$ & $ +1.33\%  $

 & ${0.4782}^{\dagger \ddagger \mathsection }$ & $ +3.73\%  $

 & ${0.0922}^{\dagger \ddagger \mathsection }$ & $ +4.03\%  $

 & ${0.3049}^{\dagger \ddagger \mathsection }$ & $ +7.05\%  $

& 19778/27983/15828

\\
\texttt{KESM (ES)}
 & ${0.6528}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +2.24\%  $

 & ${0.4769}^{\dagger \ddagger \mathsection }$ & $ +3.46\%  $

 & ${0.0920}^{\dagger \ddagger \mathsection }$ & $ +3.82\%  $

 & ${0.3026}^{\dagger \ddagger \mathsection }$ & $ +6.27\%  $

& 18619/29973/14997

\\
\texttt{KESM (EW)}
 & ${0.6767}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +5.98\%  $

 & ${0.5018}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +8.86\%  $

 & ${0.0989}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +11.57\%  $

 & ${0.3277}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +15.08\%  $

& 22805/26436/14348

\\ \hline

\texttt{KESM}
 & $\bf{0.6866}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +7.53\%  $

 & $\bf{0.5080}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +10.21\%  $

 & $\bf{0.1010}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +13.93\%  $

 & $\bf{0.3335}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +17.10\%  $

& 23290/26883/13416

\\ \hline \hline

\end{tabular}

\vspace{0.2cm}

\begin{tabular}{l|lr|lr|lr|lr|c}
\hline \hline
\multicolumn{10}{c}{\textbf{Semantic Scholar}} \\ \hline
\bf{Method}& \multicolumn{2}{c|}{\bf{Precision@1}}& \multicolumn{2}{c|}{\bf{Precision@5}}& \multicolumn{2}{c|}{\bf{Recall@1}}& \multicolumn{2}{c|}{\bf{Recall@5}}&\bf{W/T/L}\\ \hline

\texttt{Frequency}
& ${0.3944}$ & $ -9.99\%  $

 & ${0.2560}$ & $ -11.38\%  $

 & ${0.1140}$ & $ -12.23\%  $

 & ${0.3462}$ & $ -13.67\%  $

& 11155/64455/24390
 \\
\texttt{Page Rank}
& ${0.3946}^{\dagger }$ & $ -9.94\%  $

 & ${0.2561}^{\dagger }$ & $ -11.34\%  $

 & ${0.1141}^{\dagger }$ & $ -12.11\%  $

 & ${0.3466}^{\dagger }$ & $ -13.57\%  $

& 11200/64418/24382

\\ \hline

\texttt{LeToR}
& $0.4382$ & --  & $0.2889$ & --  & $0.1299$ & --  & $0.4010$ & --  & --/--/-- \\ \hline

\texttt{KESM (E)}
& ${0.4793}^{\dagger \ddagger \mathsection }$ & $ +9.38\%  $

 & ${0.3192}^{\dagger \ddagger \mathsection }$ & $ +10.51\%  $

 & ${0.1432}^{\dagger \ddagger \mathsection }$ & $ +10.26\%  $

 & ${0.4462}^{\dagger \ddagger \mathsection }$ & $ +11.27\%  $

& 27735/56402/15863

\\
\texttt{KESM (ES)}
& ${0.4901}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +11.84\%  $

 & ${0.3161}^{\dagger \ddagger \mathsection }$ & $ +9.43\%  $

 & ${0.1492}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +14.91\%  $

 & ${0.4449}^{\dagger \ddagger \mathsection }$ & $ +10.95\%  $

& 28191/54084/17725

\\
\texttt{KESM (EW)}
 & ${0.5097}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +16.31\%  $

 & ${0.3311}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +14.63\%  $

 & ${0.1555}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +19.77\%  $

 & ${0.4671}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +16.50\%  $

& 32592/50428/16980

\\ \hline

\texttt{KESM}
 & $\bf{0.5169}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +17.96\%  $

 & $\bf{0.3336}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +15.47\%  $

 & $\bf{0.1585}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +22.09\%  $

 & $\bf{0.4713}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +17.53\%  $

& 32420/52090/15490

\\ \hline \hline
\end{tabular}

\end{table*}


\section{Evaluation Results}
The section first presents the overall evaluation results on the entity salience task and the ad hoc search task. Then it provide analyses about the advantages of modeling salience over counting frequency and case studies that demonstrate the connections between semantic text understanding and search accuracy.

\subsection{Entity Salience Performance}
%=====to discuss
	% KESM's individual components E, W, S
	% Table description
    % baseline performance
    	% Frequency, PR and LeToR
    % E VS PR, the gain of kernels    
    % +S: more stable and easier to converge
    % +W: another gains: we need word-entity duet
    % Full model: effectiveness and robustness
    
    % Compare the frequency performance, and the relative gains on the two data sets, lead to experiment 3.
%==================
The overall results in the entity salience task are in Table~\ref{tab:overall_salience}. 
All the relative performances (percentages) and document level \textbf{W}in/\textbf{T}ie/\textbf{L}oss are compared with \texttt{LeToR}, the feature-based state-of-the-art~\cite{dunietz2014new,dojchinovski2016crowdsourced}. 
% the word kernel votes, $\Phi(e, \mathbb{W})$, and the semantic memory that enriches the entity embedding with the description CNN. The groups of evidences used by  \texttt{KESM} versions are in the parentheses. \texttt{KESM (EWS)} is the full model.
Among the baselines, \texttt{Frequency} provides reasonable estimations of entity salience. 
The most frequent entity is often salient to the document; the Precision@1 is rather high, especially on New York Times. 
\texttt{Page Rank} does not perform well on both corpora. Although its embeddings are trained by the salience labels, it barely improves \texttt{Frequency}. 
\texttt{LeToR}, on the other hand, significantly improves both precision and recall of \texttt{Frequency}~\cite{dunietz2014new}, which is expected as it has much richer features from various sources.
% The Parsing and Coreference features provide more stable frequency counts, while position and embedding votes reflect entity importance. 

The full model \texttt{KESM} outperforms all baselines significantly. Its improvements over \texttt{LeToR} are more than $15\%$ on all evaluations, with the only exception on Precision@1 in New York Times. 
The improvements are also robust: About twice as many documents are improved (Win) than hurt (Loss). The neural salience model learned end-to-end is also rather different than manual features; \texttt{KESM} provided different salience estimations on half documents compared to \texttt{LeToR}.

Besides the full model \texttt{KESM}, its variants with partial evidence are also evaluated: Those marked with (E) include the entity kernels; those with (W) include word kernels; those with (S) incorporated semantic memories. All versions of \texttt{KESM} include the entity kernel group, which is the most essential evidence.

The full version (\texttt{KESM}) performs the best among all variations, showing that all components contributed.
Individually, \texttt{KESM (E)} outperforms all baselines. Compared to \texttt{Page Rank}, its only difference is that instead of raw cosine similarities,
\texttt{KESM (E)} uses kernel filters, which are much more powerful in modeling the interaction patterns and lead to completely different results than \texttt{Page Rank}~\cite{K-NRM}.
\texttt{KESM (EW)} always significantly outperform \texttt{KESM (E)}, showing the interactions with words are also important. 
However, the semantic memory (S) provides mixed impacts on the accuracy of \texttt{KESM}. A possible reason is that the Freebase descriptions might be too general and the training data is large enough for the entity embeddings to ``memorize'' the domain specific semantics. Nevertheless, we do find that adding the external semantics makes the model converges faster and more stably.


These results demonstrated that \texttt{KESM} is much more effective in modeling entity salience than counting frequency either directly (\texttt{Frequency}) or through complexed linguistic or semantic processes (\texttt{LeToR}). Section~\ref{sec:analysis} will further investigate the limitations of frequency signals and the advantages of modeling salience. 


\begin{table*}[t]
\centering
\caption{
Ad hoc search accuracy of \texttt{KESM} when used as ranking features in learning to rank.
Relative performances over \texttt{LeToR} are shown in the percentages. W/T/L are the number of queries a method improves, does not change, or hurts, compared with \texttt{LeToR}. $\dagger$, $\ddagger$, $\mathsection$, and $\mathparagraph$ mark the statistically significant improvements over \texttt{BOE-TagMe}$^\dagger$, \texttt{LeToR}$^\ddagger$, \texttt{ESR}$^\mathsection$, and \texttt{ESR+LeToR}$^\mathparagraph$. \texttt{Base} is the base retrieval model, which is SDM in ClueWeb09-B and language model in ClueWeb12-B13.
% All supervised ranking models used RankSVM with the same hyper-parameters and cross validation splits. 
Best results are marked \textbf{bold}.
\label{tab:overall_ranking}
}

\begin{tabular}{l|lr|lr|c||lr|lr|c}
\hline \hline
 & \multicolumn{5}{c||}{\bf{ClueWeb09-B}}
 & \multicolumn{5}{c}{\bf{ClueWeb12-B13}}
 \\ \hline 
\multicolumn{1}{c|}{\bf{Method}} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline

\texttt{Base}
 & ${0.2496}$ & $ -5.26\%  $

 & ${0.1387}$ & $ -10.20\%  $

& 62/38/100
 & ${0.1060}$ & $ -12.02\%  $

 & ${0.0863}$ & $ -6.67\%  $

& 35/22/43


\\
\texttt{BOE-TagMe}
 & ${0.2294}$ & $ -12.94\%  $

 & ${0.1488}$ & $ -3.63\%  $

& 74/25/101

 & ${0.1173}$ & $ -2.64\%  $

 & ${0.0950}$ & $ +2.83\%  $

& 44/19/37

\\
\hline

\texttt{LeToR}
 & $0.2635$ & --  & $0.1544$ & --  & --/--/--
 & $0.1205$ & --  & $0.0924$ & --  & --/--/--\\

\texttt{ESR}
 & ${0.2695}^{\dagger }$ & $ +2.30\%  $

 & ${0.1607}$ & $ +4.06\%  $

& 80/39/81
 & ${0.1166}$ & $ -3.22\%  $

 & ${0.0898}$ & $ -2.81\%  $

& 30/23/47

\\ \hline
\texttt{KESM}
 & ${0.2799}^{\dagger }$ & $ +6.24\%  $

 & ${0.1663}$ & $ +7.68\%  $

& 85/35/80
 & ${0.1301}^{\dagger \mathsection }$ & $ +7.92\%  $

 & $\bf{0.1103}^{\ddagger \mathsection \mathparagraph }$ & $ +19.35\%  $

& 43/25/32
\\
\hline
\hline
\texttt{ESR+LeToR}
 & ${0.2791}^{\dagger \ddagger }$ & $ +5.92\%  $

 & ${0.1613}$ & $ +4.46\%  $

& 91/34/75

 & ${0.1281}$ & $ +6.30\%  $

 & ${0.0951}$ & $ +2.87\%  $

& 45/24/31


\\
\texttt{KESM+LeToR}
 & $\bf{0.2993}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +13.58\%  $

 & $\bf{0.1797}^{\dagger \ddagger \mathsection \mathparagraph }$ & $ +16.38\%  $

& 98/35/67
& $\bf{0.1308}^{\dagger \mathsection }$ & $ +8.52\%  $

 & ${0.1079}^{\ddagger \mathsection \mathparagraph }$ & $ +16.77\%  $

& 43/23/34


\\
\hline \hline

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
\caption{
Ranking performances of \texttt{LeToR}, \texttt{ESR}, and \texttt{KESM} with title or body field individually.
Relative performances (percentages) and Win/Tie/Loss are calculated by comparing with \texttt{LeToR} on the same field.
$\dagger$ and $\ddagger$ mark the statistically significant improvements over \texttt{LeToR}$^\dagger$ and \texttt{ESR}$^\ddagger$, also on the same field.
Best results are marked \textbf{bold}.
\label{tab:field_ranking}
}

\begin{tabular}{l|lr|lr|c||lr|lr|c}
\hline \hline
 & \multicolumn{5}{c||}{\bf{ClueWeb09-B}}
 & \multicolumn{5}{c}{\bf{ClueWeb12-B13}}
 \\ \hline 
\multicolumn{1}{c|}{\bf{Method}} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L} &
\multicolumn{2}{c|}{\bf{NDCG@20}} &
\multicolumn{2}{c|}{\bf{ERR@20}} &
\bf{W/T/L}
\\ \hline
\texttt{LeToR-Title}
  & ${0.2584}$ & $ -3.51\%  $

 & ${0.1460}$ & $ -5.16\%  $

& 83/48/69

 & ${0.1187}$ & $ +6.23\%  $

 & ${0.0894}$ & $ +3.14\%  $

& 41/23/36

 \\
\texttt{ESR-Title}
 & $0.2678$ & --  & $0.1540$ & --  & --/--/--
 & $0.1117$ & --  & $0.0867$ & --  & --/--/--

\\ \hline
\texttt{KESM-Title}
 & $\bf{0.2780}^{\dagger }$ & $ +3.81\%  $

 & $\bf{0.1719}^{\dagger \ddagger }$ & $ +11.64\%  $

& 91/46/63

 & $\bf{0.1199}$ & $ +7.36\%  $

 & $\bf{0.0923}$ & $ +6.42\%  $

& 35/28/37


\\ \hline \hline

\texttt{LeToR-Body}
 & ${0.2550}$ & $ +0.48\%  $

 & ${0.1427}$ & $ -3.44\%  $

& 80/46/74

 & ${0.1115}$ & $ +4.61\%  $

 & ${0.0892}$ & $ -3.51\%  $

& 36/30/34
\\
\texttt{ESR-Body}
& $0.2538$ & --  & $0.1478$ & --  & --/--/--
& $0.1066$ & --  & $0.0924$ & --  & --/--/--
\\ \hline
\texttt{KESM-Body}
  & $\bf{0.2795}^{\dagger \ddagger }$ & $ +10.13\%  $

 & $\bf{0.1661}^{\dagger \ddagger }$ & $ +12.37\%  $

& 96/39/65

  & $\bf{0.1207}^{\ddagger }$ & $ +13.25\%  $

 & $\bf{0.1057}^{\dagger \ddagger }$ & $ +14.44\%  $

& 43/24/33
\\
\hline \hline


\end{tabular}
\end{table*}



\subsection{Ranking Performance}

%===to discuss
	% overall performance
    	% KESM VS ESR
        % KESM+LeToR VS ESR+LeToR
        	%common set up
            %more additional information
        % shows that salience is better than frequency
        	% despite the knowledge transfer
     % per field performance
     	% no needs on title
        % better on body as expected, 10+\%
        % perform very differently with ESR, not only LeToR
        	% very different information

	% the task differences, the knowledge transfer, lead to the case study in experiment 4
Table~\ref{tab:overall_ranking} lists the evaluation results in the ad hoc search task.
The three supervised methods, \texttt{LeToR}, \texttt{ESR}, and \texttt{KESM}, all use the exact same learning to rank model (RankSVM) and only differ in their features.
% \texttt{LeToR} uses standard word-based features~\cite{xiong2017duet}; \texttt{ESR} uses the entity-based exact and soft match features using bag-of-entities (frequency-based) and pre-trained knowledge graph embeddings (TransE); \texttt{KESM} uses the normalized kernel votes that estimate the salience of query entities in the document. 
The effectiveness of \texttt{ESR} features and \texttt{KESM} features are also evaluated when combined with word-based features (\texttt{ESR+LeToR} and \texttt{KESM+LeToR}), which is a very common way to include new features in search engines.

On both ClueWeb09-B and ClueWeb12-B13, \texttt{KESM} features are more effective than both \texttt{LeToR} features and \texttt{ESR} features. On ClueWeb12-B13, \texttt{KESM} individually outperforms both supervised baselines significantly by $8-20\%$. On ClueWeb09-B, \texttt{KESM} provides more novel ranking signals and \texttt{KESM-LeToR} greatly improves the ranking accuracy than \texttt{ESR+LeToR}. The fusion on ClueWeb12-B13 (\texttt{KESM+LeToR}) is not as successful perhaps because of the limited ranking labels on ClueWeb12-B13.

Ranking is a complicated task with many factors influencing the final results. 
To better investigate the effectiveness of entity salience in search, we further evaluates the three supervised rankers on different document fields. Table~\ref{tab:field_ranking} lists the ranking accuracies of \texttt{LeToR}, \texttt{ESR}, and \texttt{KESM}, when only features from the document titles (\texttt{Title}) or the document body texts (\texttt{Body}) are used.

The per-field results reveal that the advantages of \texttt{KESM} are more significant and robust on the body field than on the title field.
Document titles are often short and more carefully written. Intuitively the handful entities mentioned in a title are all salient, despite spam.
The power of entity salience model is to find the importance of entities in document content---the \texttt{KESM} features learned from the New York Times corpus do reflect this semantic understanding capability on the body field features.

The W/T/L ratios in Table~\ref{tab:overall_ranking} and Table~\ref{tab:field_ranking} demonstrated that the entity salience features provide novel ranking signals.
Entity-oriented search was known to dramatically change the word-based rankings; both \texttt{ESR} and \texttt{KESM} perform rather differently with \texttt{LeToR} in Table~\ref{tab:overall_ranking}.
In addition, as shown in Table~\ref{tab:field_ranking}, the salience-based features also perform very different with \texttt{ESR}'s frequency-based features. Although both used the same entity annotations, \texttt{KESM} differs with \texttt{ESR} on $80\%$ queries and improved the majority of them.


A significant finding in our experiments is the connections of  entity salience  and  ad hoc search .
Entity salience was considered as a semantic text understanding task~\cite{dunietz2014new} while ad hoc search is a core information retrieval task.
The two tasks are different in many aspects: different focuses, different labels, different domains, and different applications. Despite these practical differences, 
the knowledge learned from entity salience labels are also effective on ad hoc search.
% Intuitively, the ability to better estimating entity salience improves the semantic text understanding in search engines which should lead to better search accuracy. 
Previously it is less common to see such connections between semantic text understanding tasks and information retrieval tasks.
Our case studies in Section~\ref{sec:case} will further discuss how \texttt{KESM} bridges the gap between semantic text understanding and search.



\begin{figure*}[t]
\centering
\begin{subfigure}{0.24\textwidth}
\includegraphics[width=\textwidth]{nyt_doclen.pdf}
\caption{New York Times \label{fig:nyt_doclen}}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\includegraphics[width=\textwidth]{s2_doclen.pdf}
\caption{Semantic Scholar \label{fig:s2_doclen}}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\includegraphics[width=\textwidth]{cw09_doclen.pdf}
\caption{ClueWeb09-B \label{fig:cw09_doclen}}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\includegraphics[width=\textwidth]{cw12_doclen.pdf}
\caption{ClueWeb12-B13 \label{fig:cw12_doclen}}
\end{subfigure}

\caption{Performances on documents at different lengths.
New York Times and Semantic Scholar documents are partitioned based on their lengths (number of words). ClueWeb queries are partitioned based on the average length of their candidate documents from base retrieval. 
The x-axes are the maximum length of the documents and their percentile of each document/query group. 
The y-axes are the Precision@5 (New York Times and Semantic Scholar) or NDCG@20 (ClueWeb09-B and ClueWeb12-B13).
The histograms are ordered the same as the legends.
\label{fig:doclen}
}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\textwidth]{nyt_entity_dist.pdf}
\caption{New York Times \label{fig:nyt_dist}}
\end{subfigure}
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=\textwidth]{s2_entity_dist.pdf}
\caption{Semantic Scholar \label{fig:s2_dist}}
\end{subfigure}
\caption{
The distribution of salient entities predicted by entity salience models and in the golden standard. The entities are binned by their frequencies in the testing data. The x-axes mark the percentile range of each group. The y-axes are the fraction of salient entities in each bin as predicted by the corresponding method.
The closer the predict salient entity distribution is to the golden standard, the more realistic an entity salience model is.
The histograms are ordered the same as the legends.
\label{fig:e_dist}
}
\end{figure*}


\subsection{From Frequency To Salience}
\label{sec:analysis}
%====performance VS. doc length 
	%==unstable on short documents
    %==will not be sufficient at per document level anyway (can be on corpus level or large scale query log level)
    
%====estimation distribution
	%==frequency favors head entities
        %==biased
		%==less interesting for sure
This experiment provides two analyses that show the advantage of modeling salience over counting frequency.
% The first one studies their performances on documents with different lengths. The second one studies their biases on head (frequent) entities.

\textbf{Reliability VS. Document Length.}
The reliability of frequency counts depends on the number of observations. Frequency signals can be very reliable at large scales. For example, the most frequent entities in a commercial search log or in a whole corpus probably reflect meaningful and stable trends. However, in each individual documents, the frequency signals might not be as reliable.

This analysis studies the performances of models on documents with different lengths.
In the entity salience task, we group the testing documents into five bins by their length (number of words). In the ad hoc search task, we group the testing queries by the average lengths of its candidate documents. The performances of the frequency-based method (\texttt{Frequency} in entity salience and \texttt{ESR} in ad hoc search), \texttt{LeToR}, and \texttt{KESM} in the five bins are plotted in Figure~\ref{fig:doclen}. The bins are ordered from short (left) to long (right) with their bin bounds and percentiles marked on the x-axes.

In the entity salience task, there is a clear trend that the frequency signals are less reliable on shorter documents. As shown in Figure~\ref{fig:nyt_doclen} and Figure~\ref{fig:s2_doclen}, \texttt{Frequency} performs much worse on shorter documents, \texttt{LeToR} has a similar trend with \texttt{Frequency} as the majority of its signals are frequency-based, and the advantages on \texttt{KESM} are more significant on short documents.
In ad hoc search, the correlations are less strong because the document length is the average of all candidate documents. Nevertheless, the improvements from \texttt{KESM} are again larger on shorter documents as shown in Figure~\ref{fig:cw09_doclen} and Figure~\ref{fig:cw12_doclen}.
On all four datasets, even in the longest document bin where documents have thousands of words, the frequency-based method still under-performs salience-based method: counting frequency is not sufficient in modeling texts at the document level.


\textbf{Bias Towards Head Entities.}
Another drawback of frequency-based methods is that they are biased towards more frequent (head) entities. To demonstrate this effect, Figure~\ref{fig:e_dist} groups the entities based on their frequency in the corpus and plot the distribution of salience entities predicted by each method. 

The x-axes label the percentiles of each bin.
For example, $<0.1\%$ refers to the top $0.1\%$ most frequent entities. The distribution of predicted-salient entities is marked by the y-axes. The predicted-salient entities is the top k entities with highest salience scores predicted by a method, where k is the number of salient entities in the ground truth. \texttt{Golden Standard} is the ground truth.

In both datasets, entity salience follows the power law distribution. \texttt{Golden Standard} favors the head entities much more than the tail ones. However, the frequency-based methods are even more biased towards the head entities. More than $40\%$ of \texttt{Frequency}'s salience predictions go to top $0.1\%$ entities on New York Times and about $30\%$ on Semantic Scholar goes to the top $0.1\%$. They almost doubled the ground truth distributions. Such unrealistic bias towards the head entities limits the effectiveness of frequency-based methods and also their attractiveness---the selected entities are mostly common ones. 
In comparison, the distributions of \texttt{KESM} are much more closer to the ground truth. On Semantic Scholar the two are almost identical.




\begin{table*}[th]
\caption{Examples from queries that \texttt{KESM} improved or hurt, compared to \texttt{ESR}. 
Documents are selected from those that ESR and KESM disagreed.
The descriptions are manually written to reflect the main topics of the documents. 
\label{tab:eg}
}
\begin{tabular}{c|c|l|l}
\hline \hline
\multicolumn{4}{c}{\textbf{Cases that KESM Improved}} \\ \hline

\textbf{Query} & \textbf{Query Entities}  & \textbf{ESR Preferred Document}  & \textbf{KESM Preferred Document} \\ \hline 

\multirow{2}{*}{ER TV Show} & ``ER (TV Series)" & clueweb09-enwp02-22-20096 & clueweb09-enwp00-55-07707  \\
& ``TV Program" & ``List of films without article" & ``ER ( TV series ) - Wikipedia"  \\
\hline

\multirow{2}{*}{Wind Power
} &
\multirow{2}{*}{``Wind Power
''} 
& clueweb12-0200wb-66-32730 & clueweb12-0009wb-54-01932  \\

&  & ``Home solar power systems" & ``Wind energy | Alternative Energy HQ"  \\
\hline

Hurricane Irene  
 &
 ``Hurricane Irene"
& clueweb12-0705wb-49-04059 & clueweb12-0715wb-81-29281
 \\

Flooding in Manville NJ &  ``Flood";  ``Manville, NJ" & ``Disaster funding for Hurricane Irene" & ``Videos and news about Hurricane Irene"  \\
\hline
% \end{tabular}


% \begin{tabular}{c|c|l|l}
\hline \hline
\multicolumn{4}{c}{\textbf{Cases that KESM Hurt}} \\ \hline

% \textbf{Query} & \textbf{Query Entities}  & \textbf{ESR Preferred Document}  & \textbf{KESM Preferred Document} \\ \hline 

\multirow{2}{*}{Fickle Creek Farm
} &  ``Malindi Fickle"  & clueweb09-en0003-97-27345
 & clueweb09-en0005-66-00576
  \\
& ``Stream"; ``Farm" & ``Hotels near Fickle Creak" 
& ``List of breading farms"  \\
\hline

\multirow{3}{*}{Illinois State Tax
} &
``Illinois"; 
& clueweb09-enwp01-67-20725
 & clueweb09-en0011-23-05274
  \\

&  ``State government"; 
& ``Sales taxes in the United & ``Retirement-related general  \\

& ``Tax in the US"
& States, Wikipedia''
& purpose taxes by State''
\\

\hline

 \multirow{2}{*}{Battles in the Civil War}
 &
 ``Battles"
& clueweb09-enwp03-20-07742
 & clueweb09-enwp01-30-04139
 \\

 &  ``Civil War" & ``List of American Civil War battles" & ``List of wars in the Muslim world"  \\
\hline
\end{tabular}

\end{table*}

\subsection{From Text Understanding to Search}
\label{sec:case}

% Show case studies:
% queries: ESR mistakes and KESM fixes (their top 1 ranked documents)

% Show that KESM provide better modeling of the query entity's relevance in a document than simple bin votes. One step further from ESR's soft match. Can be considered as a kind of semi or unsupervised learning.

% Show that KESM is thus more vulnerable to noisy query entities. There is also no good query level understanding yet. More query structures might be needed, which is the next generation of Information Retrieval.

The last experiment provides case studies that demonstrate how \texttt{KESM} transfers the semantic text understanding learned from salience labels to search. We first picked the queries that \texttt{KESM-body} improved or hurt compared to \texttt{ESR-body}, Then we manually examined the top ranked documents that the two methods disagreed. The queries, query entities, and disagreed documents are listed in Table~\ref{tab:eg}. 
% Three queries in either win or loss cases are selected.

The improvements from \texttt{KESM} are mainly from its ability to promote documents that actually focus on the query entities. 
As shown in the top half of Table~\ref{tab:eg}, \texttt{KESM} promotes documents where the query entities are more salient: the Wikipedia page about ER TV show, a homepage about wind power, and the new article about the hurricane. On the other hand, \texttt{ESR}'s frequency-based ranking might be confused by web pages that list a lot of movies or only partially talk about the query topic; without modeling salience, it is hard to exclude those web pages because the query entities are also mentioned frequently in them.

Interestingly, many errors \texttt{KESM} made are also due to its emphasizes on query entities. When a query entity does not align with the information need, promoting documents about it is risky. As shown in the lower half of Table~\ref{tab:eg}, ``Malindi Fickle'' is a mistakenly linked query entity; ``Civil War'' in the Muslim world is in linked to the civil war in American, and the query ``Illinois State Tax'' is search for sales tax as designated by TREC by not ``Tax in the US''.


There are also other winning or losing scenarios and not all their causes are identifiable. Nevertheless, the main trend found in our case study is \texttt{KESM}'s ability to identify whether a document emphasis the query entities or not, which is exactly the motivation of the entity salience task. 
% The synergy of \texttt{KESM} in entity salience estimation and document ranking suggests a promising future of applying semantic text understanding techniques in information retrieval tasks.

% These failure cases further confirmed \texttt{KESM}'s ability to transfer entity salience modeling performance to search accuracy.

% There remains a lot to be done in improving the semantic understanding of texts. 
% This case study demonstrated the connections between semantic text understanding and information retrieval made by entity salience modeling. It also shows the potential of future developments in semantic text understanding in improving search accuracy.
% Further developments in semantic text have the potential to further improve information retrieval tasks through entities.

% Both the winning cases and losing cases further demonstrate the connections between text understanding and search accuracy bridged by entity salience modeling---better text understanding improves search engines' ability to pick the documents more related to the query information needs. 
% While failures in the semantic part mislead the ranking system, it is promising that future progresses in semantic text representation and understanding techniques can lead to more intelligent and semantic search engines.





==> v1/Experiment.tex <==
\begin{table}[t]
\caption{Datasets used in the entity salience prediction task.
\label{tab:dataset}
}
\begin{tabular}{l|ccc|ccc}
\hline \hline
& \multicolumn{3}{c|}{\textbf{New York Times}}  & \multicolumn{3}{c}{\textbf{Semantic Scholar}}\\ \hline
& Train  & Dev   & Test & Train  & Dev   & Test \\ \hline
\# of Documents &  
526k & 64k & 64k &
800k & 100k & 100k
\\ \hline
Entities Per Doc &   
198 & 197 & 198 &
66 & 66 & 66
\\ \hline
Salience Per Doc &   
27.8 & 27.8 & 28.2 &
7.3 & 7.3 & 7.3
\\ \hline
Unique Word &
609k & 278k & 281k &
921k & 300k & 301k
\\ \hline
Unique Entity &
622k & 319k & 317k &
331k & 162k & 162k
\\ \hline 
\end{tabular}

\end{table}



\begin{table*}[t]
\caption{Entity salience features used by the LeToR baseline. The features are extracted via various natural language processing techniques, as indicated by the \textbf{Source} column.
\label{tab:feature}
}
\begin{tabular}{l|l|l}
\hline \hline
\textbf{Name} & \textbf{Description} & \textbf{Source} \\ \hline
Frequency & The frequency of the entity & Entity Linking\\ 
First Location & The location of the first sentence that contains the entity & Entity Linking \\ \hline
Head Word Count & The frequency of the entity's first head word in parsing & Dependency Parsing \\
Is Named Entity & Whether the entity is considered as a named entity & Named Entity Recognition \\
Coreference Count & The coreference frequency of the entity's mentions & Entity Coreference Resolution \\  \hline
Embedding Vote & Votes from other entities through cosine embedding similarity & Entity Embedding (Skip-gram) \\
\hline \hline
\end{tabular}
\end{table*}

\section{Experimental Methodology}
Our experiments evaluated the effectiveness \texttt{KESM} in both entity salience task and ad hoc search task. This section first describes the experimental methodologies used in the salience task and then in the ad hoc search task.

\subsection{Entity Salience Task}
The entity salience experiments mainly follow the experiment setup by Dunietz and Gillick~\cite{dunietz2014new} with some revisions to facilitate the applications in search. An additional dataset is also introduced.





\textbf{Datasets} used include \emph{New York Times} and \emph{Semantic Scholar}.

The \emph{New York Times} corpus has been used in previous work~\cite{dunietz2014new}. It includes more than half million news articles and their expert-written summarizes~\cite{sandhaus2008new}. 
Among all entities annotated to a news article, those that also appear in the summary of the article are considered as salient entities and others are not~\cite{dunietz2014new}. 

The \emph{Semantic Scholar} corpus is the scientific publications from Semantic Scholar, the academic search engine from Allen Institute for Artificial Intelligence. The full texts of the papers are not publicly available due to copyright reasons. Only the abstract and title of the paper content are made public. We treat the entities annotated to the abstract as the candidate entities of a paper and those also annotated to the title as salient.
There are more than 10 million papers index by Semantic Scholar. One million of them are randomly sampled for our experiments.

The entity annotations on both corpora are Freebase entities linked by TagMe~\cite{TagMe}, a setup widely used in entity-oriented search. 
Instead of only keeping named entities in several categories~\cite{dunietz2014new}, we keep all annotated entities in all categories to ensure coverage, which has been found very crucial in providing effective text representations~\cite{Xiong2016BOE, raviv2016document}.

The statistics of the two corpora are listed in Table~\ref{tab:dataset}. The Semantic Scholar corpus has shorter documents (paper abstracts) and a smaller entity vocabulary because its papers are mostly in the computer science and medical science domain.



% \textbf{Salience Labels:}

\textbf{Baselines:} Three baselines from previous research are compared: \texttt{Frequency}, \texttt{Page Rank}, and \texttt{LeToR}.

\texttt{Frequency}~\cite{dunietz2014new} estimates the salience of an entity by its frequency. It is a straightforward but effective baseline in many related tasks.

\texttt{PageRank}~\cite{dunietz2014new} estimates the salience score of an entity using its page rank score. 
It is also a widely used baseline in graph-based text representations~\cite{blanco2012graph}. We conduct a supervised PageRank on a fully connected graph whose nodes are the entities in the document and edges are the embedding similarities of corresponding entity pairs. The entity embeddings are configured and learned using the same pairwise loss as used in \texttt{KESM}. 

Similar to previous work~\cite{dunietz2014new}, we found \texttt{PageRank} not very effective in the entity salience task. It is hard for the model to learn anything; many times the training loss did not drop at all. The best setup we were able to find and presented in the evaluation results is to one-step random walk linearly combined with \texttt{Frequency}. It is essentially equal to an embedding-based translation model~\cite{K-NRM}

\texttt{LeToR}~\cite{dunietz2014new} is a feature-based learning to rank (entity) model. It is trained using the same pairwise loss with \texttt{KESM}, which we found more effective than the pointwise loss used in prior research~\cite{dunietz2014new}. 

We tried our best to reproduce the features used by Dunietz and Gillick~\cite{dunietz2014new}. 
As listed in Table~\ref{tab:feature}, the features are extracted by various linguistic and semantic techniques including entity linking, dependency parsing, named entity recognition, and entity coreference resolution. 
The entity embeddings are trained on the same corpus using Google's Word2vec toolkit~\cite{word2vec}; entity linking is done by TagMe; other linguistic and semantic preprocessing were done by the Stanford CoreNLP toolkit~\cite{StanfordNLP}.

Compared to Dunietz and Gillick~\cite{dunietz2014new}, we do not include the headline feature because it uses information from the expert-written summary and does not improve the performance much anyway; we also replace the head-lex feature with Embedding Vote which has similar effectiveness but more efficient.








\textbf{Evaluation Metrics:}
We use the ranking-focused evaluation metrics: Precision@\{1, 5\} and Recall@\{1, 5\}.
These ranking evaluation metrics avoid the requirement to select cutoff thresholds in the classification evaluation metrics~\cite{dunietz2014new}. The cutoff thresholds may vary in different documents and selecting proper ones can be tricky.
Statistical significances are tested by permutation test (randomization test) with $p<0.05$.


\textbf{Implementation Details:} The hyper-parameters of \texttt{KESM} are configured following popular choices or previous research.
The dimension of entity embeddings, word embeddings, and CNN filters are all set to 128.
The kernel pooling layers use one exact match kernel ($\mu=1, \sigma=1e-3$) and ten soft match kernels with $\mu$ equally splitting the cosine similarity range $[-1, 1]$, i.e. $\mu \in\{-0.9, -0.7...,0.9\}$ and $\sigma=0.1$~\cite{K-NRM}.
The length of the CNN used to encode entity description is set to 3 which is tri-gram.
The entity descriptions are fetched from Freebase. Only the first 20 words of the description is used which defines and explains the entity.
The words or entities that appear less than 2 times in the training corpus are replaced with  ``Unk\_word'' or ``Unk\_entity''.

The parameters include the embeddings $V$, the CNN weights $W^g$, the projection weights $W^s$, and the kernel weights $W^f$. They are learned end-to-end from the training data. The learning used the Adam optimizer, mini-batch with size 64, and early stopping on the development split. 
% The majority of the parameters and the main capacity of \texttt{KESM} are the entity and word embeddings $V$. 
$V$ is initialized by the word2vec of words and entities jointly trained on the training corpora~\cite{JointSem}.

With our PyTorch implementation and a typical GPU, \texttt{KESM} converges within several hours and usually only needs one pass on the training data. 
In comparison, \texttt{LeToR} takes more time to extract its features since parsing and coreference may take days to process more than half million documents.















\subsection{Ad Hoc Search Task}
\label{sec:adapt}
Our ad hoc ranking experiments follow a popular setup in recent entity-oriented search research~\cite{xiong2017duet}. The datasets and baselines in our experiments are obtained from the authors' website\footnote{http://boston.lti.cs.cmu.edu/appendices/SIGIR2017\_word\_entity\_duet/}.

\textbf{Datasets} used are those from TREC Web Track ad hoc search task, the widely used benchmarks for ad hoc search. It includes 200 queries  for the ClueWeb09 corpus and 100 queries for the ClueWeb12 corpus. The category B of the two corpora and corresponding relevance judgments are used.

All the rankings were done to re-rank the top 100 candidate documents from SDM (ClueWeb09-B) and language model (ClueWeb12-B13) from previous research~\cite{daltonentity,xiong2017duet}.
The documents were parsed by boilerpipe into title and body fields~\cite{boilerpipe}.
The queries and documents are annotated to Freebase entities by TagMe. Standard spam filtering is applied on ClueWeb09-B but not on ClueWeb12-B13~\cite{daltonentity,xiong2017duet}.

\textbf{Baselines:}
The goal of our experiments is to explore the usage of entity salience modeling in ad hoc search, instead of achieving the best ad hoc ranking accuracy. To this purpose, our experiments focus on evaluating the effectiveness of the entity salience features from \texttt{KESM} in standard learning to rank; the proper baselines are the ranking features from word-based matches (\texttt{LeToR}) and entity-based matches (\texttt{ESR}~\cite{ESR}), utilized by the same learning to rank model.
Unsupervised retrieval with words (\texttt{Base}) and entities (\texttt{BOE-TagMe}) are also included.

\texttt{Base} is the base retrieval model, which is SDM on ClueWeb09-B and language model on ClueWeb12-B.

\texttt{BOE-TagMe} is the retrieval model with bag-of-entities~\cite{Xiong2016BOE}.  
It exact-matches query and documents in the entity space and has similar effectiveness with the entity language model~\cite{raviv2016document} as they use the same information.

\texttt{LeToR} is the feature-based learning to rank with bag-of-words. Typical retrieval model features were used~\cite{xiong2017duet}.

\texttt{ESR} is the entity-based learning to rank. 
It includes both exact match and soft match signals in the entity space~\cite{ESR}. The differences with \texttt{KESM} are that it uses knowledge graph embeddings and its representation is based on entity frequency.





\textbf{Evaluation Metrics} are NDCG@20 and ERR@20, official evaluation metrics of TREC Web Tracks. Statistical significances are tested by permutation test (randomization test) with $p<0.05$.

\textbf{Implementation Details:}
As discussed in Section~\ref{sec:adapt}, we adapt the \texttt{KESM} trained on the New York Time corpus to ad hoc search by using its kernel votes as learning to rank features.
The entity salience features are combined by the same learning to rank model (RankSVM~\cite{ranksvm}) as used by \texttt{LeToR} and \texttt{ESR} with exactly the same cross validation setup~\cite{xiong2017duet}.
Similar to \texttt{ESR}, the base retrieval score is included as a feature in \texttt{KESM}.

As a result, the comparisons of \texttt{KESM} with \texttt{LeToR} and \texttt{ESR} hold out all other factors and directly investigate the effectiveness of entity salience features, in a widely used learning to rank framework.
Given the current exploration stage of semantic text understanding in information retrieval,
we believe this is more informative than mixing entity salience signals into sophisticated ranking systems such as latent space models~\cite{liu2015latent, EsdRank} and attention-based models~\cite{xiong2017duet,JointSem} where many other factors come into play.



==> v1/Introduction.tex <==
\section{Introduction}

%=======Language understanding is a long desired goal, lots of effort in text understanding, but currently there is a discrepancy, IR is still mostly simplified as bag-of-words and counting.
Understanding the semantics of texts has been a long desired goal in information retrieval. 
% Tremendous efforts have been devoted to understand language using computational linguistic and semantic techniques.
Historically, the semantic text understanding techniques such as semantic parsing and grounding did not necessarily lead to  more accurate search, while search was mostly conducted by frequency-based methods~\cite{croft2010search, liu2007letor}. 
% However, there has been a discrepancy between text understanding and information retrieval performances, and search was mostly conducted by matching and counting query words in documents.
%=======The development of Entity-oriented Search is one step forward towards search with meanings, abstract word to entity, and bring in external semantics. but still starts from entity annotation and counting
The recent developments of entity-oriented search started to address this discrepancy~\cite{KG4IRTutorial}. 
It enriches the representation of query and documents with entities from knowledge graphs~\cite{SELM, ESR} and improves ranking using semantics such as attributes and relations~\cite{daltonentity, liu2015latent, xiong2015fbexpansion, EsdRank}.  The entity-based representations and semantic signals have improved various aspects of search and moved one step forward towards the goal of ``search with meanings''~\cite{bast2016semantic, dietz2017first}.


In the entity-based text representations, the importance of an entity in the text is still determined by its frequency~\cite{hasibi2016exploiting, xiong2017duet}. However, frequency is not equal to importance:
A document centered around an entity may not explicit mention it frequently, for example, many Wikipedia articles do not repeat its title entity---the most important one---the most times. On the other hand, the most mentioned entities are also not necessarily the most important to the document's central topic, for example, they can be ``stop entities''.
Solely relying on frequency signals restricts the search to coarse and shallow text understanding and may limit the potential of semantic and intelligent information retrieval systems. 



%=======This paper moves towards better text understanding with entity salience modeling. The motivation, and how it was done previously. 
This paper focuses on improving entity-based text representation and search by modeling the importance, or \textit{salience}, of entities in documents. 
The goal of entity salience modeling is to figure out which entities are central to the main topic of a text, which is the next step towards semantic text understanding after entity linking~\cite{dunietz2014new, dojchinovski2016crowdsourced}.
% As expected, this is a rather challenging task: Previous approaches rely heavily on linguistic signals such as parsing, named entity recognition, and coreference, which are rather costly and only slightly outperform simple frequency based methods~\cite{dunietz2014new}. 
%=======how we do it in this paper.
This paper presents a Kernel Entity Salience Model (\texttt{KESM}) that models the entity salience end-to-end using neural networks.
\texttt{KESM} embeds entities annotated to a document using distributed representations, models the interactions between entities and words using the kernel pooling technique~\cite{K-NRM}, and combines the votes from kernel filters into salience scores.
% After the kernel filters convert the embedding similarities between entities and words to salience votes, \texttt{KESM} combines these votes to the entity salience score using a feed-forward layer. 
By training end-to-end using automatically generated salience labels~\cite{dunietz2014new}, \texttt{KESM} learn the interaction patterns between entities in the document to predict the salience of entities.



%=======from better text understanding to better search, the intuition and how we do it
\texttt{KESM} is also able to improve search accuracy under the framework of entity-oriented search.
% This paper further adapts the entity salience model to improve information retrieval under the framework of entity-oriented search.
% For example, a document in which the entity ``Wind Power'' is salience should be relevant to the query ``wind power''.
In this paper, we developed an adaption method that fine-tunes the pre-trained entity salience model using search relevance labels. As a result, the knowledge learned from the entity salience task is transferred to ad hoc search.
It is used to model the salience of query entities in candidate documents and provide additional ranking signals to the ranking system.
% which helps determine the document relevance, for example a document in which the entity ``Wind Power'' is salience should be relevant to the query ``wind power''.



%=======experiments in salience and in web search
Our experiments on a news corpus~\cite{dunietz2014new} and a scientific proceeding corpus~\cite{ESR} demonstrated the advantage of \texttt{KESM}. \texttt{KESM} outperforms previous frequency-based and feature-based salience models by large margins in both precision and recall.
\texttt{KESM}'s ability in better modeling entity salience is also effective in ad hoc search. 
Our experiments on TREC Web Track revealed that the entity salience signals are more effective than frequency based ranking signals.
The \texttt{KESM} pre-trained on the news corpus outperforms word-based and entity-based ranking models on ClueWeb web corpora, despite the domain differences (news versus web) and the task differences (entity salience versus ad hoc search).

%=======the finding in salience: when frequency cannot get it done
%=======observations in web search: promote documents that indeed focus more on the query entity. Shows that we connects text understanding with text retrieval.
Our analyses revealed two advantages of modeling entity salience over counting entity frequency.
First, \texttt{KESM} provides more reliable salience estimations when there is not enough frequency signals, especially on shorter documents.
% the reliability of frequency signals depends on the length of documents. On all four datasets, the advantage of \texttt{KESM} is observed on documents even longer than 5000 words but is much stronger on shorter documents where the frequency count is not as reliable.
Second, the predicted salience entities of \texttt{KESM} distributes more realistically on entities of variant frequencies, while the distribution of frequency-based predictions is rather skewed towards the most frequent entities.
% though the salient label has a long tail distribution, the distribution of frequency-based predictions is even more skewed towards the most frequent entities, while the predictions of \texttt{KESM} distributes more realistically on entities of variant frequencies. 

We also found many interesting cases when examining the document rankings provided by entity salience. The main source of \texttt{KESM} effectiveness in ranking is its ability to promote documents whose main topics are actually about the query entities and to demote those only partially mention the query entities. At the same time, the errors \texttt{KESM} made are also frequently from twisting the document ranking towards the query entities that either are mistakenly linked or  do not represent the search intent.
These case studies revealed that \texttt{KESM} does further bridges the gap between semantic text understanding and search accuracy: 
while the search accuracy may be mislead by imperfect text understanding,
better entity linking and salience modeling do improve the search accuracy significantly.

In the rest of this paper, Section 2 discusses the related work, Section 3 describes the kernel entity salience model.
% and how it is used in entity salience estimation.
Section 4 discusses how the entity salience model is adapted to ad hoc search.
Experimental methodology and results for entity salience are presented in Section 5 and Section 6. 
Those for ad hoc search are in Section 7 and Section 8. We conclude in Section 9.
% Section 9 concludes and provides future work directions.



==> v1/Related.tex <==
\section{Related Work}

%====entity-oriented search

% over view of entity-oriented search
Though the first generation of search engines was built upon structured semantic resources such as controlled vocabularies, the field later switched to full text based representations such as bag-of-words, perhaps due to the lack of coverage of the semantic resources back then and also the efficiency and low cost of bag-of-words.
However, the recent emergence of large scale general domain knowledge graphs, for example, Freebase and DBpedia, and automatic semantic grounding techniques, such as entity linking and entity search, have motivated information retrieval researchers and practitioners to revisit the applicability of the structured semantic resources in information retrieval.

After years of development, the recent progresses of utilizing knowledge graphs and semantic resources in text analysis and retrieval have provided effective approaches that improved various components of search engines. 
These developments, which have been referred as ``entity-oriented search''~\cite{KG4IRTutorial}, ``knowledge graph for information retrieval'' (KG4IR)~\cite{dietz2017first}, or more generally ``semantic search''~\cite{bast2016semantic}, can be categorized into \emph{query representation}, \emph{retrieval model}, and \emph{document representation} methods based on their primary focuses in the search pipeline.

% query expansion alike
The \emph{query representation} approaches aim to improve or expand the representation of the query using entities and their semantics from knowledge graphs.
Wikipedia have been widely used as an external and high quality corpus in query expansion, especially for noisy corpora like web corpora~\cite{xu2009query, nguyen2010combination}.
Freebase entities that being retrieved by the query through entity search or linked frequently to the retrieved documents provide additional and semantic evidence to explain the query; their descriptions are good sources of expansion terms and their types provide semantic signals to select those terms~\cite{xiong2015fbexpansion}; their attributes, relations, and appearance in the documents have also been used to extract richer learning to rank features in entity query feature expansion (EQFE)~\cite{daltonentity}.

% retrieval models
The \emph{retrieval model} methods utilize entities to build additional connections between query and documents, mainly through latent space models.
The Latent Entity Space (LES) method treats query annotations as a latent layer in the language model and uses the names and descriptions of the annotated entities to estimate the language model probabilities~\cite{liu2015latent}.
EsdRank developed a latent learning to rank model to learn the connections from query to entities and the ranking of documents from ranking labels; it also found that query annotation provides more related entities than entity search and document annotations~\cite{EsdRank}.

% text representation
	% BOE
    % SELM
    % The graph connection
    % ESR
    % Duet
The \emph{document representation} approaches further introduced the entities linked to the document into the ranking process.
The bag-of-entities model represents query and document in the entity space, in which exact match can improve both ad hoc search~\cite{raviv2016document, Xiong2016BOE} and also entity search~\cite{hasibi2016exploiting}.
More interestingly, the semantics associated with entities make soft match in the entity space effective: the relations between the query entities and the document entities help  connect the query and documents~\cite{schuhmacher2014knowledge, SELM}; Explicit Semantic Ranking (ESR) method addresses the sparsity of knowledge graph edges by encoding them to embeddings, and then soft matches the query and documents with the knowledge graph embeddings~\cite{ESR}.
The bag-of-entities representation can also be integrate with the original word-based representations; the textual fields of entities enable the cross-space matching with bag-of-words and introduce additional ranking signals~\cite{xiong2017duet}.

A major challenge in entity-oriented search is the uncertainties form the entity representations which is automatically constructed by semantic grounding technique and thus inevitably contains noise.
The noise in query entities was a major bottleneck in entity-oriented search and often had to be manually cleaned~\cite{daltonentity,SELM,liu2015latent}. Recently, Xiong et al. provided a series of models to automatically learn the importance of query entities~\cite{EsdRank, xiong2017duet} or to integrate the query entity linking process into entity-oriented search with joint modeling~\cite{JointSem}.
These methods mainly focus on addressing the linking errors in the query entities as queries are often short and ambiguous thus hard to annotate. 


%====entity salience modeling and similar efforts in summarization, etc.
% the challenge of frequency and salience
% mostly in the NLP community
On the other hand, the entity representations for the documents in entity-oriented search are mostly frequency-based, i.e. in the bag-of-entities model~\cite{ESR,SELM}.
As recently studied in the entity salience task, the frequency of an entity is not equal to its importance or centrality in the document~\cite{dunietz2014new,dojchinovski2016crowdsourced}.
Dunietz and Grllick~\cite{dunietz2014new} developed the new entity salience task using the New York Time corpus~\cite{sandhaus2008new}; they consider the entities that annotated to the expert-written summarization salient to the article and automatically constructed millions of training documents.
Dojchinovski et al. constructed a deeper study using a smaller corpus with golden standard entity annotations and crowdsource workers~\cite{dojchinovski2016crowdsourced}.
They found that crowdsource workers consider entity salience an intuitive task and that the noise in entity linking does not affect the estimation of entity salience as much as expected.
In both work, they demonstrated that a supervised model with features such as named entity recognition, parsing, and coreference is able to outperform frequency-based methods.




%====neural IR



==> v1/half_conclusion.tex <==
\section{Conclusion and Future Work}


This paper presents \texttt{KESM}, the kernel entity salience model that estimates the salience of entities in documents using neural networks.
\texttt{KESM} represents entities and words with distributed representations,  models their interactions using kernel filters, and combines the kernel scores to estimate entity salience. The external semantics of entities in the knowledge graph---their descriptions---are also incorporated to enrich entity embeddings. 
The whole model is trained end-to-end using  automatically generated entity salience labels.


In addition to the entity salience task, this paper provides an adaptation method that ranks documents by the salience of query entities in them.
It uses \texttt{KESM} to calculate the kernel scores of query entities and then combines them to salience ranking features, which describe how much focused the document is on the query entities. 
When ranking labels are limited, \texttt{KESM} can be pre-trained on large scale salience labels and its features can be used in standard learning to rank. In that case, the text understanding ability learned from the salience task is transferred to search by \texttt{KESM}.






Our experiments on two entity salience corpora, one news corpus from previous research (New York Times) and one scientific publication corpus generated by ourselves (Semantic Scholar), demonstrate the effectiveness of \texttt{KESM} in the entity salience task.
Significant and robust improvements are observed over frequency and feature-based methods. 
Compared to those baselines, \texttt{KESM} behaves more stable on shorter documents and select more novel salient entities; its kernel interaction model is also more powerful than the raw embedding similarities as used by PageRank.
Overall, \texttt{KESM} is a much stronger model with richer sources of evidence and more powerful architecture.



Our experiments on the ad hoc search task were conducted on the TREC Web Track queries and two ClueWeb corpora. In both corpora, the salience features provided by the \texttt{KESM} trained on the New York Times corpus outperform both typical word-based ranking features and a frequency-focused entity-based ranking features, despite various differences between the salience task and the ranking task. The advantages of the salience features are also more observed on the document body field than on the title field, as on the latter perhaps all entities are salient anyway.


% Our exploration concluded with case studies that evince \texttt{KESM}'s ability to transfer the semantic text understanding capability learned from from salience labels to  search.
% We found that \texttt{KESM} influences the document ranking by promoting the documents that actually emphasize the query entities. 
% This effect leads to improvements when the query entities align well with the information needs.

Our case study on the winning and losing queries of \texttt{KESM} shows that the influences the salience features have on the document rankings are indeed that they help distinguish those documents in which the query entities are the core topic from those where the query entities are only partial to the central meanings or just mentioned multiple times. 
Interestingly, this effect leads to both winning cases---better text understanding leads to more accurate search results---and also losing cases, because when the query entities do not align well with the underlying search intent, emphasizing them does mislead the document ranking.



% Our findings point to the promising future of semantic and intelligent information retrieval where search is conducted by not only matching the query and documents but also understanding them.
% This is an underdeveloped area with a lot of future research directions.
% An immediate next step is to combine the salience signals with more advanced entity-oriented search models. For example, the attention-based ranking models can be used to handle the noisy query entities, although more complex models will require more training data~\cite{xiong2017duet}.
% Another future research direction is to better transfer the entity salience model to ad hoc search.
% As the first step, this paper directly uses the salience kernels as ranking features. One can also view \texttt{KESM} as the pre-training of a neural ranking model, in which the gaps between source and target tasks are bridged by the entity salience. It will be interesting to see how the entity-based text modeling interacts with the recent processes in word-based neural information retrieval.


 
% %frequency vs salience
% Our analyses further revealed the advantage of modeling salience over counting frequency.
% The first advantage is that the reliability of frequency signals depends on the length of documents, 
% while salience modeling performs much more stable on texts with variant lengths.
% On all four datasets of the two tasks, the improvements of \texttt{KESM} over \texttt{Frequency} is larger on shorter documents on which the frequency signal is not as reliable.
% The second advantage is that \texttt{KESM} provides a more realistic treatment on the tail entities.
% Frequency-based methods heavily favor the most frequent entities which limits their effectiveness and also attractiveness, while the saliences predicted by \texttt{KESM} are distributed across entities with different popularities similar to the ground truth.


